LiveHand: Real-time and Photorealistic Neural Hand Rendering

The human hand is the main medium through which we interact with our surroundings, making its digitization an important problem. While there are several works modeling the geometry of hands, little attention has been paid to capturing photo-realistic appearance. Moreover, for applications in extended reality and gaming, real-time rendering is critical. We present the first neural-implicit approach to photo-realistically render hands in real-time. This is a challenging problem as hands are textured and undergo strong articulations with pose-dependent effects. However, we show that this aim is achievable through our carefully designed method. This includes training on a low-resolution rendering of a neural radiance field, together with a 3D-consistent super-resolution module and mesh-guided sampling and space canonicalization. We demonstrate a novel application of perceptual loss on the image space, which is critical for learning details accurately. We also show a live demo where we photo-realistically render the human hand in real-time for the first time, while also modeling pose- and view-dependent appearance effects. We ablate all our design choices and show that they optimize for rendering speed and quality. Video results and our code can be accessed from https://vcai.mpi-inf.mpg.de/projects/LiveHand/

==> figures/shape_editing.tex <==
\begin{figure}[]
	\centering
    \includegraphics[width=\linewidth]{figures/shape_editing.png}
	\caption{Application: Shape Editing. The hand geometry can be edited without any additional retraining of the model.}
	\label{fig:shape_editing}
\end{figure}


==> sections/conclusion_old.tex <==
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
\section{Conclusion and Future Work} \label{sec:conclusions}

We presented the first neural implicit approach that can render human hands in a photorealistic manner in real-time. 
%
Our approach is carefully designed in a way to optimize the rendering quality and speed. 
%
At the heart of our method is a low-resolution NeRF rendering together with a super-resolution module that produces 3D-consistent results. 
%
Here, we showed that a novel application of the perceptual loss on the full image space is important for high-quality photorealistic rendering, which was only possible because of our design choices which made the model efficient. 
%
To ensure our model can capture pose-dependent effects, the representation is also conditioned on the MANO pose parameters.
%
We also utilize the MANO hand mesh to guide the sampling of points in 3D space to better improve the rendering speed. 
%
Results show that our method generates a wide variety of hand articulations, capturing high-frequency skin textural changes arising from skin wrinkles and hand veins.  
%
Comparison with related methods clearly shows that our approach outperforms the baselines by a significant margin.
%
In addition, we show the novel application of editing the hand geometry while keeping the texture fixed. 

%
While our work is an important milestone for the full digitization of human hands, there are still several avenues for future work. 
%
Since our work requires a MANO mesh, future work could look into improving the quality of such a mesh and corresponding pose parameters. 
%
This could include refining the geometry, possibly in an end-to-end manner. 
%
Another more strategic direction moving forward is to learn a generalizable implicit 3D morphable model of the human hands that is photoreal. This will give full access to all the hand semantics. 
%
While our approach models hand-pose dependant shadow effects, it can not model shadow as a function of any random illumination condition other than the one under the training set that was captured. We leave this modeling for future works.


==> sections/related_work2.tex <==
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
\input{tables/conceptual_comparison.tex}
%
\section{Related Works} \label{sec:related}
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
\par 
%
\textbf{Geometry Modeling.}
%
Parametric 3D morphable models map low-dimensional control variables to deforming meshes enabling easy and efficient control of the generated geometry~\cite{FLAME:SiggraphAsia2017,SMPL-X:2019,MANO:SIGGRAPHASIA:2017,alldieck2021imghum}.
%
Relevant to our work, MANO~\cite{MANO:SIGGRAPHASIA:2017} learns a parametric hand model using high-resolution 3D scans, parametrizing the mesh as a function of the hand shape and pose. 
%
Implicit geometry modeling uses a neural network to encode the geometry as an isosurface. 
%
Since the learned representation is resolution-independent, it can - in theory - be used to retrieve meshes at arbitrarily-high resolution at inference time. 
%
imGHUM~\cite{alldieck2021imghum} builds a parametric full-body model comprising of detailed body, face, and hand geometry.
%
GraspingField~\cite{GraspingField:3DV:2020} learns a signed distance function (SDF) of hand-object interaction, which fits the MANO model onto the SDF to recover the final pose estimate. 
%
However, none of the existing hand models~\cite{MANO:SIGGRAPHASIA:2017,li21piano,moon2020deephandmesh,GraspingField:3DV:2020,karunratanakul2021halo} include a component for the hand texture.
%
In contrast, our goal is to model the photorealistic hand appearance in real-time.
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
\par 
%
\textbf{Geometry and Appearance Modeling.}
%
A few approaches extend parametric mesh by complementing it with a texture map. 
%
HTML~\cite{qian2020html} builds a low-dimensional hand appearance model by applying principal component analysis (PCA) to texture maps of 51 subjects. 
%
NIMBLE~\cite{li2022nimble} uses MRI data to learn a parametric mesh model based on the bones and muscles, and uses light-stage captures to obtain the appearance maps (including albedo, normal maps, and specular maps). 
%
A PCA on the various components of appearance maps give them an appearance model. 
%
Since both HTML and NIMBLE use a linear model to compress the appearance variations to a low-dimensional space, their expressivity is severely limited.
%
For example, they lack details such as veins and colored fingernails since these are person-specific attributes.
%
% DART~\cite{gao2022dart} provides a way to overcome this limitation by releasing 325 hand-crafted 2D texture maps for blemishes, make-up, and accessories, which can be added to the hand texture. 
%
% However, since the texture map does not change based on the hand pose, these approaches can not model hand appearance as a function of hand pose. 
%
% In contrast, our neural hand model learns pose- and view-dependent appearance effects leading to increased immersiveness and photorealism.
%
Closest to our approach is LISA~\cite{corona2022lisa}, which models the hand shape and appearance using a neural implicit field. 
%
% They decompose the hand into individual bones, each of which is encoded with a separate MLP. 
%
The underlying MLPs are conditioned on pose and appearance parameters, allowing pose and appearance changes at inference.
%
However, the reconstructions lack high-frequency details, and the approach takes about one minute to render an image at $1024\times667$ pixels. 
%
On the other hand, we focus on creating a digital hand avatar in a person-specific setup and show photorealistic results in real-time. 
%
Please refer to Tab.~\ref{tab:concecptual_comparison} for a conceptual comparison of the existing hand modeling methods.
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
\par 
%

\edits{
\textbf{Other Articulated Objects.} 
%
The literature contains works for modeling other objects such as the human face ~\cite{Lombardi21,Cao22,Zheng:CVPR:2022,grassal2022neural,Gao2022nerfblendshape}, animals ~\cite{Luo22} and human body ~\cite{habermann2021,vid_based_charcs,bhatnagar2020ipnet,liu2021neural,yang2022banmo,peng2021neural,su2021nerf}. 
%
Humans hands differ in their highly articulated motions, which usually contains strong self-occlusions and pose-dependent effects. 
%
In contrast, face related methods either only handle rigid motions ~\cite{Lombardi21,Cao22,Gao2022nerfblendshape} and/or are not real-time ~\cite{grassal2022neural,Zheng:CVPR:2022,Gao2022nerfblendshape}. 
%
Methods for the human body can handle more articulated motions. 
%
The existing explicit mesh-based methods~\cite{vid_based_charcs,habermann2021,Bagautdinov21} rely on a template mesh obtained from a static scene and then learn appearance in the mesh space either by retrieval~\cite{vid_based_charcs} or by using a CNN to directly regress the texture map~\cite{habermann2021,Bagautdinov21}. 
%
The strong reliance on the template mesh has two limitations. 
%
First, if the deformed template mesh does not match the real deformation of the surface, the learned appearance will be oversmoothed and blurry. 
%
Secondly, the mesh representation is limited by its resolution, which may prevent the capture of high-quality details.
%
In addition to the aforementioned work on parametric body meshes, many approaches have studied implicit geometry modeling of the clothed human body using neural networks \cite{palafox2021npms, tiwari21neuralgif, Saito:CVPR:2021, xiu2022icon}.
%
Some approaches decompose the body into individual body parts \cite{bhatnagar2020ipnet, mihajlovic2022coap, biswas2021hipnet}, allowing a better generalization to out-of-distribution poses.
%
Due to their capabilities of modeling non-rigid clothing deformations well, implicit models are also used to model the geometry and appearance of clothed humans \cite{su2021nerf, peng2021neural, 2021narf, liu2021neural, peng2021animatable, yang2022banmo, habermann2022hdhumans}. 
%
%\ME{However, none of the existing implicit-based body reenactment methods can operate in real-time.}
%\ME{However, until now there is no method for implicit-based rendering of the human hands that runs in real-time}.
\ME{we need a new concluding statement based on our findings on implicit-based body models}
%
}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

